Simplistic Collection and Labeling Practices Limit the Utility of Benchmark Datasets for Twitter Bot Detection

Accurate bot detection is necessary for the safety and integrity of online platforms. It is also crucial for research on the influence of bots in elections, the spread of misinformation, and financial market manipulation. Platforms deploy infrastructure to flag or remove automated accounts, but their tools and data are not publicly available. Thus, the public must rely on third-party bot detection. These tools employ machine learning and often achieve near perfect performance for classification on existing datasets, suggesting bot detection is accurate, reliable and fit for use in downstream applications. We provide evidence that this is not the case and show that high performance is attributable to limitations in dataset collection and labeling rather than sophistication of the tools. Specifically, we show that simple decision rules -- shallow decision trees trained on a small number of features -- achieve near-state-of-the-art performance on most available datasets and that bot detection datasets, even when combined together, do not generalize well to out-of-sample datasets. Our findings reveal that predictions are highly dependent on each dataset's collection and labeling procedures rather than fundamental differences between bots and humans. These results have important implications for both transparency in sampling and labeling procedures and potential biases in research using existing bot detection tools for pre-processing.

==> caverlee-without-created-tree.tex <==
\begin{tikzpicture}[
    node/.style={%
      draw,
      rectangle,
    },
  ]

    \node [node] (A) [draw, align=center]{Followings greater than 232?};
    \path (A) ++(-125:\nodeDist) node [node] (B) [draw, align=center] {NUMBER of tweets greater than 63};
    \path (A) ++(-55:\nodeDist) node [node] (C) [draw, align=center] {number of tweets greater than 1000};
    \path (C) ++(-110:\nodeDist) node [node] (D) {A};
    \path (C) ++(-70:\nodeDist) node [node] (E) {B};
    \path (B) ++(-110:\nodeDist) node [node] (F) {NumerOfFollowings greaterthan 66.50};
    \path (B) ++(-70:\nodeDist) node [node] (G) {HUMAN};

    \path (D) ++(-110:\nodeDist) node [node] (H) {A};
    \path (D) ++(-70:\nodeDist) node [node] (I) {B};
    \path (E) ++(-110:\nodeDist) node [node] (J) {C};
    \path (E) ++(-70:\nodeDist) node [node] (K) {D};

    \path (F) ++(-110:\nodeDist) node [node] (L) {A};
    \path (F) ++(-70:\nodeDist) node [node] (M) {B};



    \draw (A) -- (B) node [left,pos=0.5] {NO}(A);
    \draw (A) -- (C) node [right,pos=0.5] {YES}(A);
    \draw (C) -- (D) node [left,pos=0.5] {NO}(A);
    \draw (C) -- (E) node [right,pos=0.5] {YES}(A);
    \draw (B) -- (F) node [left,pos=0.5] {NO}(A);
    \draw (B) -- (G) node [right,pos=0.5] {YES}(A);
\end{tikzpicture}



%    \begin{tabular}{l}
% %     \textbf{caverlee without CreatedAt} \\
% %      |--- NumerOfFollowings <= 232.50\\
% %     |   |--- NumberOfTweets <= 63.50\\
% %     |   |   |--- NumerOfFollowings <= 66.50\\
% %     |   |   |   |--- weights: [1626.00, 781.00] class: 0\\
% %     |   |   |--- NumerOfFollowings >  66.50\\
% %     |   |   |   |--- weights: [176.00, 1446.00] class: 1\\
% %     |   |--- NumberOfTweets >  63.50\\
% %     |   |   |--- NumerOfFollowings <= 92.50\\
% %     |   |   |   |--- weights: [6567.00, 208.00] class: 0\\
% %     |   |   |--- NumerOfFollowings >  92.50\\
% %     |   |   |   |--- weights: [3707.00, 835.00] class: 0\\
% %     |--- NumerOfFollowings >  232.50\\
% %     |   |--- NumberOfTweets <= 1085.50\\
% %     |   |   |--- NumberOfTweets <= 402.50\\
% %     |   |   |   |--- weights: [339.00, 9255.00] class: 1\\
% %     |   |   |--- NumberOfTweets >  402.50\\
% %     |   |   |   |--- weights: [525.00, 2135.00] class: 1\\
% %     |   |--- NumberOfTweets >  1085.50\\
% %     |   |   |--- NumerOfFollowings <= 863.50\\
% %     |   |   |   |--- weights: [1740.00, 430.00] class: 0\\
% %     |   |   |--- NumerOfFollowings >  863.50\\
% %     |   |   |   |--- weights: [744.00, 2685.00] class: 1\\
% %     Accuracy: 0.8806024096385542\\
% %     Precision 0.9087254670134783\\
% %     Recall: 0.8639838129496403\\
% %     F1: 0.8857900195920247\\
% % \end{tabular}

==> datasets-table-components.tex <==
\begin{table}[t]
\label{tab:constit-datasets}
\caption{Publicly available individual benchmark datasets for bot detection.}

    \begin{tabular}{l r r r} 
    \toprule 
Component dataset & Ref. & Humans & Bots
\\
\midrule

\data{botwiki-2019} & \cite{yang2020scalable} & 0 & 698 \\
\data{celebrity-2019} & \cite{yang2019arming} & 5918 & 0 \\
\data{the-fake-project-2015} & \cite{cresci2015fame} & 469 & 0 \\
\data{elezioni-2015} & \cite{cresci2015fame} & 1488 & 0 \\
\data{fake-followers-2015} & \cite{cresci2017the} & 0 & 3351 \\
\data{genuine-accounts-cresci} & \cite{cresci2017the} & 3474 & 0 \\
\data{social-spambots-1} & \cite{cresci2017the} & 0 & 991 \\
\data{social-spambots-2} & \cite{cresci2017the} & 0 & 3457 \\
\data{social-spambots-3} & \cite{cresci2017the} & 0 & 464 \\
\data{traditional-spambots-yang} & \cite{yang2013empirical} & 0 & 1000 \\
\data{genuine-accounts-yang} & \cite{yang2013empirical} & 10000 & 0 \\
\data{traditional-spambots-2} & \cite{cresci2017the} & 0 & 100 \\
\data{traditional-spambots-3} & \cite{cresci2017the} & 0 & 403 \\
\data{traditional-spambots-4} & \cite{cresci2017the} & 0 & 1128 \\
\data{political-bots-2019} & \cite{yang2019arming} & 0 & 62 \\
\data{pronbots-2019} & \cite{yang2019arming} & 0 & 17882 \\
\data{vendor-purchased-2019} & \cite{yang2019arming} & 0 & 1087 \\
    \end{tabular}
    
\end{table}




==> leaveoneout.tex <==
\begin{tabular}{@{}lll@{}} \toprule
Dataset left out & Acc./F1 & Depth \\ \midrule
twibot-2020 & 0.45/0.18 & 1 \\
botometer-feedback-2019 & 0.65/0.40 & 1 \\
cresci-rtbust-2019 & 0.55/0.36 & 1 \\
gilani-2017 & 0.56/0.12 & 1 \\
cresci-2017 & 0.78/0.84 & 1 \\
cresci-2015 & 0.91/0.94 & 1 \\
cresci-stock-2018 & 0.65/0.66 & 1 \\
yang-2013 & 0.32/0.21 & 1 \\
\end{tabular}

==> relatedwork.tex <==
% \begin{enumerate}
%     % \item Taxonomy of bot detection techniques:
%     % \begin{enumerate}
%     %     \item Deep learning
%     %     \item Regression / random forests
%     %     \item Types of features: network stats; NLP
%     %     \item Goals: 1-off bots or botnets
%     % \end{enumerate}
% \end{enumerate}
Although we focus on the limitations of sophisticated machine learning models and large feature sets in this paper, there may be other challenges to the utility of existing bot detection tools.
%
For example, manual labels of human and automated accounts may be difficult, especially as social bots become more similar to humans.


==> results-summary-table-data_presentation.tex <==
\small
\begin{tabular}{@{}p{0.28\columnwidth}llllrr@{}} \toprule
% & \multicolumn{2}{c}{Shallow decision tree (SDT)} & \multicolumn{2}{c}{State of the art (SOTA)} & \multicolumn{2}{c}{SDT $-$ SOTA}\\ \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
% Dataset & Accuracy \textit{(depth)} & F1 \textit{(depth)} & Accuracy & F1 & Accuracy & F1 \\ \midrule
Dataset & SDT & Depth & SOTA & SDT - SOTA \\ 
(approx. size) & Acc./F1/bal.\ acc.\ &   &  & Acc./F1 \\ \midrule
\data{twibot-2020} \;\;\, ($10^3$) & 0.82/0.86/0.80  & 1 & \cite{feng2022heterogeneity-aware} & -0.05/-0.03 \\
\data{feedback-2019} ($10^2$)  & 0.80/0.55/0.69  & 3 & \cite{guo2022social} & -0.01/-0.15 \\
\data{rtbust-2019}  \;\;\, ($10^3$)& 0.71/0.73/0.71  & 4 & \cite{mazza2019rtbust} & -0.22/-0.14 \\
\data{pan-2019}  \;\;\;\;\;\;\;\;  ($10^3$)& 0.92/0.91/0.92  & 2 & \cite{geng2021satar} & -0.03/-0.04 \\
\data{midterm-2018} \, ($10^4$) & 0.97/0.98/0.95  & 1 & \cite{giorgi2021characterizing} & -0.01/\;\;--- \\
\data{stock-2018}\;\;\;\;\;\, ($10^4$) & 0.80/0.83/0.80  & 3 & \;\;---\;\; & \;\;---\;\;\,/\;\;--- \\
\data{cresci-2017} \;\;\, ($10^4$) & 0.98/0.98/0.97  & 1 & \cite{kudugunta2018deep} & -0.02/-0.02 \\
\data{gilani-2017} \;\;\, ($10^3$) & 0.77/0.72/0.76  & 3 & \cite{gilani2020classification} & -0.09/-0.11 \\
\data{cresci-2015} \;\;\, ($10^3$) & 0.98/0.98/0.98  & 3 & \cite{cresci2015fame} & -0.01/-0.01 \\
\data{yang-2013} \;\;\;\;\;\; ($10^4$) & 0.96/0.71/0.79  & 4 & \cite{yang2013empirical} & -0.03/-0.19 \\
\data{caverlee-2011} ($10^4$) & 0.91/0.91/0.90  & 2 & \cite{lee2011a} & -0.08/-0.07 \\


\end{tabular}

==> robustnesschecks.tex <==
\begin{enumerate}
    \item Create a classifier that performs well on all or many datasets. Test using leave-one-out validation, where one is a dataset
    \item Are most of the problems related to old papers? Confirm this is a recent phenomenon by removing papers written >3 years ago or reweighting and show results are same
    \item Are most of the problems related to lesser cited papers? Confirm results with papers with >50 citations etc.?
    \item Google scholar citations are inaccurate. Also check analysis using publisher's metric if they have one
    \item Is it lower-prestige venues that are doing most of the publishing of problematic papers?
\end{enumerate}

==> too-3a-table.tex <==

\setlength\tabcolsep{0pt}
\begin{tabular}{r *{8}{M{0}{1}{round-precision=2}{3em} }}
				
		
				
botometer\_feedback\_2019\_one\_hot&0.7230215827338129&0.49743589743589745&0.5289291882556131&0.5352941176470588&0.5337706511175899&0.5293577981651376&0.5331773127753304&0.422\\
cresci\_2015\_one\_hot&0.5215827338129496&0.9776923076923076&0.719055843408175&0.5&0.5042921930677032&0.49036697247706423&0.5368942731277533&0.82\\
cresci\_2017\_one\_hot&0.6258992805755396&0.6761538461538461&0.9684801381692574&0.5205882352941177&0.49044379656624554&0.5220183486238532&0.5200991189427313&0.584\\
cresci\_rtbust\_2019\_one\_hot&0.5467625899280576&0.5728205128205128&0.25115141047783535&0.7352941176470589&0.6431810819565922&0.49311926605504586&0.6013215859030837&0.8255\\
cresci\_stock\_2018\_one\_hot&0.4136690647482014&0.4864102564102564&0.7435233160621761&0.5882352941176471&0.8019922254616132&0.48027522935779815&0.5195484581497798&0.597\\
gilani\_2017\_one\_hot&0.5719424460431655&0.4958974358974359&0.4798503166378814&0.4970588235294118&0.4893909944930353&0.7293577981651376&0.47990088105726875&0.4855\\
twibot\_2020\_one\_hot&0.5&0.502051282051282&0.5038860103626943&0.5014705882352941&0.5113378684807256&0.5082568807339449&0.7830396475770925&0.6075\\
yang\_2013\_one\_hot&0.5215827338129496&0.8074358974358974&0.643062751871042&0.5&0.49991901522513765&0.4926605504587156&0.5148678414096917&0.7835\\
\rotz{} & 
\rotz{\rotatebox{-50}{botometer\_feedback\_2019\_one\_hot}} & 
\rotz{\rotatebox{-50}{cresci\_2015\_one\_hot}} & 
\rotz{\rotatebox{-50}{cresci\_2017\_one\_hot}} & 
\rotz{\rotatebox{-50}{cresci\_rtbust\_2019\_one\_hot}} & 
\rotz{\rotatebox{-50}{cresci\_stock\_2018\_one\_hot}} & 
\rotz{\rotatebox{-50}{gilani\_2017\_one\_hot}} & 
\rotz{\rotatebox{-50}{twibot\_2020\_one\_hot}} & 
\rotz{\rotatebox{-50}{yang\_2013\_one\_hot}}	
			\end{tabular}%\par\bigskip
		


==> twibot-tree.tex <==
\begin{tikzpicture}[
    node/.style={%
      draw,
      rectangle,
    },
  ]

    \node [node] (A) {Verified?};
    \path (A) ++(-120:\nodeDist) node [node] (B) {bot};
    \path (A) ++(-60:\nodeDist) node [node] (C) {human};

    \draw (A) -- (B) node [left,pos=0.5] {NO}(A);
    \draw (A) -- (C) node [right,pos=0.5] {YES}(A);

\end{tikzpicture}
